Exploiting Out-of-band Motion Sensor Data to De-anonymize Virtual Reality Users

Virtual Reality (VR) is an exciting new consumer technology which offers an immersive audio-visual experience to users through which they can navigate and interact with a digitally represented 3D space (i.e., a virtual world) using a headset device. By (visually) transporting users from the real or physical world to exciting and realistic virtual spaces, VR systems can enable true-to-life and more interactive versions of traditional applications such as gaming, remote conferencing, social networking and virtual tourism. However, as with any new consumer technology, VR applications also present significant user-privacy challenges. This paper studies a new type of privacy attack targeting VR users by connecting their activities visible in the virtual world (enabled by some VR application/service) to their physical state sensed in the real world. Specifically, this paper analyzes the feasibility of carrying out a de-anonymization or identification attack on VR users by correlating visually observed movements of users' avatars in the virtual world with some auxiliary data (e.g., motion sensor data from mobile/wearable devices held by users) representing their context/state in the physical world. To enable this attack, this paper proposes a novel framework which first employs a learning-based activity classification approach to translate the disparate visual movement data and motion sensor data into an activity-vector to ease comparison, followed by a filtering and identity ranking phase outputting an ordered list of potential identities corresponding to the target visual movement data. Extensive empirical evaluation of the proposed framework, under a comprehensive set of experimental settings, demonstrates the feasibility of such a de-anonymization attack.

==> alg.tex <==

\begin{algorithm}[H]
	\small
	\caption{Correlation Algorithm.}
	\label{alg:keystroke-detection}
	\begin{algorithmic}[1]
		\State  \textbf{Input:}
		\State \hskip 1em  $video[]$  \Comment{Video's activity-vectors series}
		\State \hskip 1em  $ motion[]$ \Comment{Motion's activity-vectors series}
		\State \hskip 1em  $t$ \Comment{Filtering Threshold}
		\State \textbf{Output: } 
		\State \hskip 1em $ranked[]$ \Comment{Ranked list of correlated motion/video indexes with maximum Spearman's rank correlation coefficient}
		\Procedure{Correlate}{}%
		
		
		\State $correlated[]$ \Comment{Maps motion indexes to correlated  video indexes} %
		\State $unranked[]$ \Comment{Unranked list of correlated motion/video indexes with maximum Spearman's rank correlation coefficient}
		
		
		
		\For{ $i$ in range($video.size() - 1$)}
			\For{ $j$ in range($motion.size() - 1$)}
				\If{$HammingDistance(video[i], motion[j]) < t$ }
				\State $correlated[i].append(j)$
				\EndIf
			\EndFor
		\EndFor
		
		\For{ $i$ in range($video.size() - 1$)}
			\For{$j$ in range($correlated[i].size() - 1$)}
			\State $m_{idx} = correlated[i][j]$  \Comment{motion index}
			\State $maxSpearman = max(Spearman(video[i], motion[m_{idx}]))$
			\State $unranked[i].append(\{maxSpearman, m_{idx}\})$
			\EndFor
			\State $ranked[i] = unranked[i].sort() $ 
			\Comment{ sorted based on Spearman’s rank correlation coefficient}
		
		\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\amjad{we need to reference the alg}

==> experimentSetup.tex <==
\section{Experimental Setup}
\label{sec:setup}

This section covers the details of the experiments conducted during our study under different action-set scenarios. Lastly, we provide details on the creation and usage of the simulated environment that will we be used to gain insights in \cref{sec:eval}.

\subsection{Actions and Sources}
\label{subsec:worlds}
Firstly, we discuss the specifics on which types of action data was collected from the participants in both the real and virtual reality (VR) worlds. 
We chose VRchat \cite{s} as our VR environment mainly due to its popularity. It is estimated that VRChat contains 7.2 million user, 30,000 daily concurrent users, and 70,000 daily users. Those numbers fluciate where in the month of July 2022 there were more than 200,000 daily users. 


In this study, actions are pre-defined gestures possible through head, arm, palm, leg movements or by using them in a combined fashion. The details of the individual actions performed by the participants are available in \cref{tab:activities}. The actions were mimicked in the virtual world application using controllers paired with an Oculus Quest 2 VR headset. The resulting motion was captured at 20ms sampling rate using motion sensors from smartwatches (TicWatch 2) worn by the participants on their wrists along with a smartphone (Moto G7 Play) placed their pockets. Additionally, the actions were visually recorded in the real world using a Go Pro 4 camera \nisha{will check model}, and in the virtual world with the help of OBS Studio \cite{} and  inbuilt Oculus cast options from different adversarial perspectives covered in the next subsection. \amjad{Figure showing all the adversaries and maybe phone locations would be good.}



\subsection{Experimental Settings}

We divide our experiments into four main segments, which can be seen in \cref{tab:setup}. Both E1 and E2 take place in VRChat home world, the default location when someone joins the VRChat. We place four models in the room at four corners shown in \cref{s} that records visual data. Additionally, we have a fifth avatar that follows the participant around. 

In E1 the participant stays at a mirror (shown in \cref{d}) and performs the pre-determined actions from \cref{tab:activities}. The participants wear two smartwatches that capture imu data from both wrists, and the phone is placed in one of the four pockets (back/front right/left pockets). We repeat the E1 four times for each pocket where the phone is placed. We repeated four times because we didn't want to bias our data by placing four phones at once as it felt unnatural to the participants and might affect how they interacted/acted. The smartwatches did not affect the participants; thus, we collected both at once. In E1 we wanted to collect data to evaluate our framework when participants produce the same actions. 

However, in E2 we wanted uncontrolled actions and evaluated our framework when the participants acted naturally. E2 itself is split into two parts; the first is asking the participants to get familiar with using VR by observing themself while facing the mirror without any movement. Typically this is the first data we collect from participants as it introduces those who have never used VR or VRChat on the controllers. The second part in E2 is that we give them the flexibility to roam freely around the world and interact however they wish. Additionally, we collected data from a different world. To compare the impact of different worlds, we create a different setup in one of the popular public worlds, "The Black Cat". Due to its popularity, there are other real-life users that our participants could interact with and thus act even more naturally then roaming in the private world. 

E3 collects data solely from the motion sensors in the real world. There is no virtual reality interaction. We collect data using similar setups of pockets and watches as E1 and E2. We asked participants to do actions that happen in real life. More specifically: Fiddling with an object, walking, running, talking on the phone, browsing/fiddling with the phone, and picking up items from the table and floor. Those activities simulate some activities that a person might be doing daily. We want to inject this motion data collected in E3 to E1 and study how effective how the framework is in not confusing regular real-life actions as virtual actions. 

Finally, E4 happens solely in the virtual world. We set up cameras in different virtual worlds and started recording. E4 is meant to populate our video data with more users from the wild.

\subsection{Adversarial Perspectives}
\amjad{The following subsections 5.3 to end could be removed in my opinion}
Adversaries were twofold in the VR world: one moving adversary who was friends with the target, and four stationary adversaries who were friends with the moving adversary but not the target. \nisha{Need to add reason for why two --  needed to build a 3D model}. The latter stationary adversaries were later strategically placed in the chosen VRChat worlds unbeknownst to the target.\nisha{Might add a figure for showing placement of adversaries.}. We later analyze how different visual perspectives affect the privacy of the target user in the VR world in \cref{sec:eval}.

\subsubsection {Stationary Adversary}
\subsubsection {Moving Adversary - Stalker}
\subsubsection {Target or Victim}

\begin{table}[]
\caption{List of controlled actions performed by participants in the real and virtual reality worlds. The \textit{italicized} actions were not part of the controlled action-set.}
\label{tab:activities}
\begin{adjustbox}{width=0.47\textwidth}
\begin{tabular}{|l|ll|} 
\toprule
\multicolumn{1}{|l|}{\textbf{Action Types}} & \multicolumn{1}{l}{\textbf{Action Description}} & \\ 
\toprule
Head-based  
 & Looking \{left, right, up, down\} &      \\
 & Rotating the head in \{clockwise, anti-clockwise\} directions &      \\
 \hline
Arm-based 
 & Raising \{left, right, both\} arms in \{forward, upward, sideward\} directions &      \\
 & Rotating \{left, right, both\} arms in \{clockwise, anti-clockwise\} directions &      \\
 & Stretching arms \{forward, upward, sideward\} &     \\
 \hline
Palm-based 
 & Handshaking with \{left, right, both\} arms &      \\
 & Waving with \{left, right, both\} arms in \{forward, upward\} directions  &      \\
 & Thumbs up and down with \{left, right, both\} arms forward &      \\
 & Clapping with hands forward &     \\
 \hline
Leg-based 
 & Stepping along \{left, right, forward, backward\} directions &      \\
 & Walking diagonally towards \{left, right, forward, backward\} directions &      \\
 & Raising \{left, right\} knee &      \\
 \hline
Combination-based
 &\{Twisting hip, turning body around\} in \{clockwise, anti-clockwise\} directions &      \\
 & Crouching or squatting, Jumping up and down &      \\
 & Sitting on the \{floor, chair\} &      \\
 & \textit{Exploring \{public, private\} instances} &      \\
 & \{Walking, running\} in \{straight, zig-zag\} paths &      \\
 & \{Talking, browsing\} smartphone in \{portrait, landscape\} modes &      \\
 & Fiddling with an object &      \\
 & Picking up objects placed on the \{floor, table\} &      \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

\subsection{Action-Set Scenarios}
Next, we describe the characteristics of action-sets used for analysis. Action-sets are a group of similar category of actions performed in different worlds. All action-sets were repeated four times during which the smartphone was placed in one of the four pant pockets. \cref{tab:setup} covers the data sources used during the different action-set scenarios we considered for our analysis. At a high level, the experiments consist of controlled, uncontrolled, and simulated actions. During the controlled experiments, the recruited participants were asked to perform a pre-defined set of actions and activities in different worlds described in \cref{subsec:worlds}. Conversely, during the uncontrolled experiments, the participants had control of their actions with minimal influence. On the other hand, the simulation-related experiments generated supplementary data for training the data models and generate additional analysis scenarios not covered in the other experiments. 


\begin{table}[]
\caption{An overview of the data sources used to collect and record different types of action-sets from target (participants) across different experimental setups in our study. \nisha{change experiment keywords}}
\label{tab:setup}
\begin{adjustbox}{width=0.48\textwidth}
\begin{threeparttable}[b]
\begin{tabular}{l|c|cc|cc|}
\cline{2-6}
\multicolumn{1}{c|}{} & \textbf{Action} & \multicolumn{2}{c|}{\textbf{Video Feeds}} & \multicolumn{2}{c|}{\textbf{Motion Sensors}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Action-Sets*}} & \textbf{Characteristics} & \multicolumn{1}{c|}{\textbf{3rd Person View}} & \textbf{1st Person View} & \multicolumn{1}{c|}{\textbf{Smartwatch}} & \textbf{Smartphone} \\ \hline
\multicolumn{1}{|l|}{E1: $VR_{cbase}$} & Pre-determined & \multicolumn{1}{c|}{\ding{51}} & \ding{51} & \multicolumn{1}{c|}{\ding{51}} & \ding{51} \\ \hline
\multicolumn{1}{|l|}{E2: $VR_{start}$} & Uncontrolled & \multicolumn{1}{c|}{\ding{55}} & \ding{51} & \multicolumn{1}{c|}{\ding{51}} & \ding{51} \\ \hline
\multicolumn{1}{|l|}{E2: $VR_{roam}$} & Uncontrolled & \multicolumn{1}{c|}{\ding{51}} & \ding{51} & \multicolumn{1}{c|}{\ding{51}} & \ding{51} \\ \hline
\multicolumn{1}{|l|}{E3:  $RW_{cbase}$} & Pre-determined & \multicolumn{1}{c|}{\ding{55}} & \ding{55} & \multicolumn{1}{c|}{\ding{51}} & \ding{51} \\ \hline
\multicolumn{1}{|l|}{E4: $VR_{ubase}$} & Uncontrolled & \multicolumn{1}{c|}{\ding{51}} & \ding{55} & \multicolumn{1}{c|}{\ding{55}} & \ding{55} \\ \hline
\end{tabular}
\begin{tablenotes}
\item * VR - Virtual Reality, RW - Real World.
\item \ding{51} The corresponding data was recorded live during the study.
\item \ding{55} The corresponding data was \textbf{not} recorded.
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}


==> fig-abstract.tex <==


\begin{abstract}

Virtual Reality (VR) is an exciting new consumer technology which offers an immersive audio-visual experience to users through which they can navigate and interact with a digitally represented 3D space (i.e., a \emph{virtual world}) using a headset device. By (visually) transporting users from the real or physical world to exciting and realistic virtual spaces, VR systems can enable true-to-life and more interactive versions of traditional applications such as gaming, remote conferencing, social networking and virtual tourism. However, as with any new consumer technology, VR applications also present significant user-privacy challenges. This paper studies a new type of privacy attack targeting VR users by connecting their activities visible in the virtual world (enabled by some VR application/service) to their physical state sensed in the real world. Specifically, this paper analyzes the feasibility of carrying out a \emph{de-anonymization} or \emph{identification} attack on VR users by \emph{correlating} visually observed movements of users' avatars in the virtual world with some auxiliary data (e.g., motion sensor data from mobile/wearable devices held by users) representing their context/state in the physical world. To enable this attack, this paper proposes a novel framework which first employs a learning-based activity classification approach to translate the disparate visual movement data and motion sensor data into an \emph{activity-vector} to ease comparison, followed by a filtering and identity ranking phase outputting an ordered list of potential identities corresponding to the target visual movement data. Extensive empirical evaluation of the proposed framework, under a comprehensive set of experimental settings, demonstrates the feasibility of such a de-anonymization attack.

\end{abstract}
